Self-driving car safety quantification via component-level analysis

In this paper, we present a rigorous modular statistical approach for arguing safety or its insufficiency of an autonomous vehicle through a concrete illustrative example. The methodology relies on making appropriate quantitative studies of the performance of constituent components. We explain the importance of sufficient and necessary conditions at the component level for the overall safety of the vehicle as well as the cost-saving benefits of the approach. A simple concrete automated braking example studied illustrates how separate perception system and operational design domain statistical analyses can be used to prove or disprove safety at the vehicle level.

==> figure_template.tex <==
\begin{figure}[h]
\begin{subfigure}[b]{0.5\textwidth}
  \centering{}
  \includegraphics[width=\textwidth]{{plots/plot_??.png}}
  \caption{\(p_c = ???\) and \(\alpha = ???\)}
  %\label{fig:p1}
  \centering{}
\end{subfigure}%  
  \begin{subfigure}[b]{0.5\textwidth}
    \centering{}
  \includegraphics[width=\textwidth]{{plots/plot_???.png}}
  \caption{\(\lambda_c = ???\) and \(\alpha = ???\)}
  %\label{fig:lambda1}
  \end{subfigure}
  
\begin{subfigure}[b]{0.5\textwidth}
  \centering{}
  \includegraphics[width=\textwidth]{{plots/plot_???.png}}
  \caption{\(p_c = ??\) and \(\alpha = ???\)}
  %\label{fig:p2}
\end{subfigure}  
  \begin{subfigure}[b]{0.5\textwidth}
    \centering{}
  \includegraphics[width=\textwidth]{{plots/plot_???.png}}
  \caption{\(\lambda_c = ???\) and \(\alpha = ???\)}
  %\label{fig:lambda2}
  \centering{}
\end{subfigure}
\caption{Required sample sizes to achieve a probability of 80\% of successfully
  establishing bounds at different underlying values of distance over-estimation
  and obstacle intensities. See Figure~\ref{fig:pandlambda}.
\end{figure}

==> img/detection_picture.tex <==
\begin{tikzpicture}
  \path [fill=green] (0.5,0) -- (9.5,0) to (0.5,0) -- (9.5,9.5) -- (9.5,0) ;
  \path [fill=red]  (0.5,0) -- (9.5,9.5 ) to (9.5,9.7) -- (0.5,9.7)--(0.5, 9.7);
  \draw [thick, <-]  (0,9.7) node [left] {e}  -- (0,0);
  \draw [thick, <-] {(-0.2,0)} -- (9.7,0) ;
  \draw [thick, <->] (0.5,- 0.56)--(9.5, -0.56);
  \node at (5, -0.75) {$\alpha$};
  \draw [thick]  (0.5,0) -- (9.7,9.7) ;
  \node at (5.5, 2.5)  {Succesful detection};
  \node at (3.5, 5.5)  {Unsuccesful detection};
  \draw [dashed, thick] (3.5, 9.7) -- (3.5,0);
  \draw [dashed, thick] (0.5, 9.7) -- (0.5,-0.1) node [below] {c};
  \draw [dashed, thick] (6.5, 9.7) -- (6.5,0);
  \draw [dashed, thick] (9.5, 9.7) -- (9.5,-0.1) node [below] {$d_b$};	
\end{tikzpicture}

